A Novel Explainable Artificial Intelligence Model in Image Classification problem

In recent years, artificial intelligence is increasingly being applied widely in many different fields and has a profound and direct impact on human life. Following this is the need to understand the principles of the model making predictions. Since most of the current high-precision models are black boxes, neither the AI scientist nor the end-user deeply understands what's going on inside these models. Therefore, many algorithms are studied for the purpose of explaining AI models, especially those in the problem of image classification in the field of computer vision such as LIME, CAM, GradCAM. However, these algorithms still have limitations such as LIME's long execution time and CAM's confusing interpretation of concreteness and clarity. Therefore, in this paper, we propose a new method called Segmentation - Class Activation Mapping (SeCAM) that combines the advantages of these algorithms above, while at the same time overcoming their disadvantages. We tested this algorithm with various models, including ResNet50, Inception-v3, VGG16 from ImageNet Large Scale Visual Recognition Challenge (ILSVRC) data set. Outstanding results when the algorithm has met all the requirements for a specific explanation in a remarkably concise time.

==> ref.tex <==
XAI methods:
1. LIME (Local Interpretable Model-agnostic Explanations):
- LIME paper: https://arxiv.org/pdf/1602.04938.pdf
2. SHAP(SHapley Additive exPlanation) Values:
- SHAP paper:
A Unified Approach to Interpreting Model
Predictions
https://arxiv.org/abs/1705.07874
- https://christophm.github.io/interpretable-ml-book/shapley.html#shapley
3. CAM (Classification Activation Mapping)
- CAM repo: https://github.com/zhoubolei/CAM
- CAM paper: https://arxiv.org/pdf/1512.04150.pdf
4. XAI tutorial
- https://xaitutorial2020.github.io/raw/master/slides/aaai_2020_xai_tutorial.pdf

Evaluation XAI: 
- Evaluation XAI through Neural backdoor: https://arxiv.org/abs/2009.10639
- Towards a Rigorous Evaluation of XAI Methods on Time Series: 
https://arxiv.org/abs/1909.07082
- A Multidisciplinary Survey and Framework for Design and Evaluation of Explainable AI Systems: https://arxiv.org/pdf/1811.11839.pdf
- General: https://github.com/SinaMohseni/Awesome-XAI-Evaluation

References Format:
https://en.wikibooks.org/wiki/LaTeX/Bibliography_Management

==> ref1.tex <==
https://arxiv.org/pdf/2005.01831.pdf
